Exact sensitivity analysis of Markov reward processes via algebraic geometry

We introduce a new approach for deterministic sensitivity analysis of Markov reward processes, commonly used in cost-effectiveness analyses, via reformulation into a polynomial system. Our approach leverages cylindrical algebraic decomposition (CAD), a technique arising from algebraic geometry that provides an exact description of all solutions to a polynomial system. While it is typically intractable to build a CAD for systems with more than a few variables, we show that a special class of polynomial systems, which includes the polynomials arising from Markov reward processes, can be analyzed much more tractably. We establish several theoretical results about such systems and develop a specialized algorithm to construct their CAD, which allows us to perform exact, multi-way sensitivity analysis for common health economic analyses. We develop an open-source software package that implements our algorithm. Finally, we apply it to two case studies, one with synthetic data and one that re-analyzes a previous cost-effectiveness analysis from the literature, demonstrating advantages of our approach over standard techniques. Our software and code are available at: \url{https://github.com/mmaaz-git/markovag}.

==> synthetic_cad.tex <==
\begin{forest}
[{}, phantom
[{$p_1_1 = 0$}
	[{$0 < p_1_2 < 1$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 - 3 p_{2 2}}{p_{1 2}}$}]
					[{$r_2 > \frac{3 - 3 p_{2 2}}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = \frac{- 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} - r_{1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} - r_{1} + 3}{p_{1 2}}$}]
				]
				[{$r_1 = - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{- 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{- 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = \frac{- 3 p_{1 2} p_{2 1} - p_{2 1} r_{1} + 3 p_{2 1}}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} p_{2 1} - p_{2 1} r_{1} + 3 p_{2 1}}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{- 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{- 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 - 3 p_{1 2}}{p_{1 2}}$}]
					[{$r_2 > \frac{3 - 3 p_{1 2}}{p_{1 2}}$}]
				]
				[{$0 < r_1 < 3 - 3 p_{1 2}$}
					[{$r_2 = \frac{- 3 p_{1 2} - r_{1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 2} - r_{1} + 3}{p_{1 2}}$}]
				]
				[{$r_1 = 3 - 3 p_{1 2}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 3 - 3 p_{1 2}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
	[{$p_1_2 = 1$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = 0$}
					[{$r_2 = 3 - 3 p_{2 2}$}]
					[{$r_2 > 3 - 3 p_{2 2}$}]
				]
				[{$0 < r_1 < \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3$}]
					[{$r_2 > - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3$}]
				]
				[{$r_1 = \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 - 3 p_{2 2}}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = 3 - 3 p_{2 1}$}]
					[{$r_2 > 3 - 3 p_{2 1}$}]
				]
				[{$0 < r_1 < 3 - 3 p_{2 1}$}
					[{$r_2 = - 3 p_{2 1} - r_{1} + 3$}]
					[{$r_2 > - 3 p_{2 1} - r_{1} + 3$}]
				]
				[{$r_1 = 3 - 3 p_{2 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 3 - 3 p_{2 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = - 3 p_{2 1} - 3 p_{2 2} + 3$}]
					[{$r_2 > - 3 p_{2 1} - 3 p_{2 2} + 3$}]
				]
				[{$0 < r_1 < \frac{- 3 p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = - 3 p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3$}]
					[{$r_2 > - 3 p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3$}]
				]
				[{$r_1 = \frac{- 3 p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{- 3 p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
]
[{$0 < p_1_1 < 1$}
	[{$p_1_2 = 0$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 3 - 3 p_{1 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 3 - 3 p_{1 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 3 - 3 p_{1 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 3 - 3 p_{1 1}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
	[{$0 < p_1_2 < 1 - p_{1 1}$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{1 2} p_{2 1} - r_{1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{1 2} p_{2 1} - r_{1} + 3}{p_{1 2}}$}]
				]
				[{$r_1 = - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{1 2}}$}]
				]
				[{$0 < r_1 < \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - p_{2 1} r_{1} + 3 p_{2 1}}{p_{1 2}}$}]
					[{$r_2 > \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} - p_{2 1} r_{1} + 3 p_{2 1}}{p_{1 2}}$}]
				]
				[{$r_1 = \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} \cdot \left(1 - p_{2 1}\right) - 3 p_{1 1} - 3 p_{1 2} p_{2 1} + 3 p_{2 1}}{p_{2 1}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{1 2} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{1 2} + 3}{p_{1 2}}$}]
				]
				[{$0 < r_1 < - 3 p_{1 1} - 3 p_{1 2} + 3$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{1 2} - r_{1} + 3}{p_{1 2}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{1 2} - r_{1} + 3}{p_{1 2}}$}]
				]
				[{$r_1 = - 3 p_{1 1} - 3 p_{1 2} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > - 3 p_{1 1} - 3 p_{1 2} + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
	[{$p_1_2 = 1 - p_{1 1}$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{1 1}}$}]
				]
				[{$0 < r_1 < \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{1 - p_{1 1}}$}]
				]
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) + 3}{1 - p_{1 1}}$}]
				]
				[{$0 < r_1 < - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) + 3$}
					[{$r_2 = \frac{- 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - r_{1} + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{- 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - r_{1} + 3}{1 - p_{1 1}}$}]
				]
				[{$r_1 = - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) + 3$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} + 3}{1 - p_{1 1}}$}]
				]
				[{$0 < r_1 < \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{1 - p_{1 1}}$}]
					[{$r_2 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} - r_{1} \cdot \left(1 - p_{2 2}\right) + 3}{1 - p_{1 1}}$}]
				]
				[{$r_1 = \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > \frac{3 p_{1 1} p_{2 2} - 3 p_{1 1} - 3 p_{2 1} \cdot \left(1 - p_{1 1}\right) - 3 p_{2 2} + 3}{1 - p_{2 2}}$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
]
[{$p_1_1 = 1$}
	[{$p_1_2 = 0$}
		[{$p_2_1 = 0$}
			[{$0 < p_2_2 < 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$0 < p_2_1 < 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$0 < p_2_2 < 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
			[{$p_2_2 = 1 - p_{2 1}$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
		[{$p_2_1 = 1$}
			[{$p_2_2 = 0$}
				[{$r_1 = 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
				[{$r_1 > 0$}
					[{$r_2 = 0$}]
					[{$r_2 > 0$}]
				]
			]
		]
	]
]
]
\end{forest}
